Real-Time Neural-Enhancement for Online Cloud Gaming

Online Cloud gaming demands real-time, high-quality video transmission across variable wide-area networks (WANs). Neural-enhanced video transmission algorithms employing super-resolution (SR) for video quality enhancement have effectively challenged WAN environments. However, these SR-based methods require intensive fine-tuning for the whole video, making it infeasible in diverse online cloud gaming. To address this, we introduce River, a cloud gaming delivery framework designed based on the observation that video segment features in cloud gaming are typically repetitive and redundant. This permits a significant opportunity to reuse fine-tuned SR models, reducing the fine-tuning latency of minutes to query latency of milliseconds. To enable the idea, we design a practical system that addresses several challenges, such as model organization, online model scheduler, and transfer strategy. River first builds a content-aware encoder that fine-tunes SR models for diverse video segments and stores them in a lookup table. When delivering cloud gaming video streams online, River checks the video features and retrieves the most relevant SR models to enhance the frame quality. Meanwhile, if no existing SR model performs well enough for some video segments, River will further fine-tune new models and update the lookup table. Finally, to avoid the overhead of streaming model weight to the clients, River designs a prefetching strategy that predicts the models with the highest possibility of being retrieved. Our evaluation based on real video game streaming demonstrates River can reduce redundant training overhead by 44% and improve the Peak-Signal-to-Noise-Ratio by 1.81dB compared to the SOTA solutions. Practical deployment shows River meets real-time requirements, achieving approximately 720p 20fps on mobile devices.

==> ablation.tex <==
This section provides additional explanations for the settings used in the previous sections.
\subsection{The importance of different patches}
\label{sec.patch_pruning}
% 在这个章节, 我们比较了进行数据过滤是否会对训练效果造成损失.
% 我们将一帧分为多个32x32大小的补丁,只对于边缘得分大于阈值的补丁(即画面较为复杂)进行微调.与之相对的,是使用所有的数据进行模型训练.我们比较了两种训练模式的表现已经训练代价,具体如表所示.
% 实验结果说明了通过对待训练图片的合理选择,可以在保证图片恢复效果相近(PSNR下降大约 0.1dB)的情况下,减少约50%的数据量,即减少一半的训练开销.

\begin{table*}
\centering
\caption{Comparison of PSNR with different data overfitting methods.}
\begin{tabular}{ccccccccc}
\toprule
\multicolumn{2}{c}{Method} & CSGO & DiabloIII & Dota2 & FIFA17 & H1Z1 & Hearthstone \\
\midrule
\multicolumn{2}{c}{Generic} & 27.20 & 28.87 & 27.80 & 25.14 & 28.94 & 27.45\\
\cline{1-2}
\multirow{4}{*}{Overfitting} & All patch & \color{red}{28.11}  & \color{red}{31.68} & \color{red}{30.07} & \color{red}{26.33} & \color{red}{30.54} & \color{red}{30.63}\\
~ & Patch-pruning  & \color{blue}{28.01} & \color{blue}{31.42} & \color{blue}{30.01} & \color{blue}{26.25} & \color{blue}{30.34} & \color{blue}{30.56}\\
\cline{2-2}
~ & $\triangle_{PSNR}$ & 0.10 & 0.26 & 0.06 & 0.08 & 0.20 & 0.07\\
~ & $\triangle_{patch}$ & 7313/17000 & 4797/17000 & 9070/17000 & 7716/17000 & 3865/17000 & 11506/17000\\
\bottomrule
\\
\toprule
~ & ~ &  HeroesOfTheStorm & LoL & ProjectCars & PU & StarCraftII & WoW \\
\midrule
\multicolumn{2}{c}{Generic} & 24.53  & 25.84  & 27.25 & 29.97 & 28.45 & 25.16\\
\cline{1-2}
\multirow{4}{*}{Overfitting} & All patch & \color{red}{27.41}  & \color{red}{29.18} & \color{red}{28.63} & \color{red}{33.54} & \color{red}{30.28} & \color{red}{26.59}\\
~ & Patch-pruning & \color{blue}{27.27} & \color{blue}{29.09} & \color{blue}{28.52} & \color{blue}{33.34} & \color{blue}{30.19} & \color{blue}{26.41}\\
\cline{2-2}
~ & $\triangle_{PSNR}$ & 0.14 & 0.09 & 0.11 & 0.20 & 0.09 & 0.18\\
~ & $\triangle_{patch}$ & 9928/17000 & 5953/17000 & 8727/17000 & 3258/17000 & 11752/17000 & 7078/17000 \\
\bottomrule
\end{tabular}
\label{tbl.patch_pruning}
\end{table*}

We compare the importance of different patches and whether data filtering would result in a loss of training effectiveness for super-resolution. We chose NAS\cite{yeo2018NAS} as the super-resolution model, and the upscaling factor is set to 4. We use the \emph{Part1} of \emph{GVSET} as the dataset and divide the LR frame into multiple patches for training whose size is 32x32. The fitting performance is also tested on the \emph{Part1} of \emph{GVSET}. Two data overfitting methods are compared. The first method involves fine-tuning only those patches with edge scores greater than the threshold $\lambda$, indicating that these patches are more complex. We set the threshold $\lambda$ to 10. The second approach involves training the model using all available data. We use a generic super-resolution model trained on DIV2K\cite{DIV2K} as the baseline.

The performance and training costs of these two data preprocessing are shown in \autoref{tbl.patch_pruning}. The red represents the best, and the blue represents the second. We use $\triangle_{PSNR}$ to represent the difference in PSNR between the two methods and $\triangle_{patch}$ to represent the change in data volume before and after pruning. Even though pruning the data leads to a performance drop of approximately 0.1dB, it is still significantly better than the baseline, with an average improvement of around 2.06 dB. This suggests that the remaining data is more important. The experimental results demonstrate that by judicious selection of training images, it is possible to reduce the data volume by approximately 50\%. This is crucial for lowering training overhead with additional GPU loads, such as cloud gaming.

\subsection{Frame or patch embedding}
% 在之前的实验中,我们将图片切片而不是以帧进行特征计算并进行聚类.
% 在本节中,我们比较了以图像块和图像帧计算特征,对于算法表现的影响.两种方法除了计算特征的单位不同以外,其余参数一致.
In Algorithm \ref{alg.model_encoder} and \ref{alg.online_schedluer}, we divide frames into patches rather than computing features per frame. In this ablation study, we compare the impact of calculating patch and frame-level features on the performance of \awRe. We chose NAS\cite{yeo2018NAS}, WDSR\cite{yu2020wdsr}, and EDSR\cite{lim2017edsr} as the super-resolution model. The upscaling factor is set to 4. Aside from the difference in the unit for the algorithms, all other parameters are kept consistent with those in Section \ref{sec.eval.compare_with_SOTA}.

\begin{table}
\centering
\caption{Comparison of PSNR of \awRe~ with various units on different SR backbones.}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule
Model & \multicolumn{2}{c}{Method} & Heroes & ProjectCars & PU & WoW \\
\midrule
\multirow{3}{*}{NAS} & \multicolumn{2}{c}{Generic} & 24.44 & \color{blue}29.10 & \color{blue}25.06 & 26.24 \\
\cline{2-3}
~ &\multirow{2}{*}{\awRe} & Frame & \color{blue}26.37 & 28.81 & 24.82 & \color{blue}27.62\\
~ & ~ &  Patch & \color{red}26.46 & \color{red}29.30 & \color{red}25.44 & \color{red}28.26\\
\hline
\multirow{3}{*}{WDSR} & \multicolumn{2}{c}{Generic} & 24.27 & 29.04 & 25.02 & 26.82 \\
\cline{2-3}
~ &\multirow{2}{*}{\awRe} &  Frame & \color{blue}26.59 & \color{blue}29.26 & \color{blue}25.06 & \color{blue}27.84\\
~ & ~ & Patch & \color{red}26.68 & \color{red}29.60 & \color{red}25.52 & \color{red}28.42\\
\hline
\multirow{3}{*}{EDSR} & \multicolumn{2}{c}{Generic} & 24.40 & \color{blue}29.12 & \color{blue}25.05 & 26.90 \\
\cline{2-3}
~ &\multirow{2}{*}{\awRe} & Frame & \color{blue}26.98 & 28.69 & 24.75 & \color{blue}28.05\\
~ & ~ &  Patch & \color{red}27.05 & \color{red}29.43 & \color{red}25.41 & \color{red}28.96\\
\bottomrule
\end{tabular}}
\label{tbl.frame_embedding}
\end{table}

% 具体实验结果如表所示,可以看到按帧特征向量进行聚类的效果远远不如按补丁进行聚类.按图像特征选择的重用模型的表现甚至不如通用模型.这是因为图像块的粒度远低于帧,按块的粒度计算相似度更为准确,这与视频压缩中的块的概念类似.
The results of this comparison are shown in \autoref{tbl.frame_embedding}. The best results are represented in red, and the second best in blue. The results indicate that calculating based on frame features performs significantly worse than based on patches. The enhancement quality is even lower than a generic model when using frame-level features for the algorithms. This is due to the high diversity in cloud gaming and the fact that the granularity of patches is much lower than that of frames, resulting in more accurate feature extraction. The approach of dividing frames into patches is similar to using blocks in video compression, such as in the H.264 codec\cite{sullivan2005h264}. This comparison demonstrates the importance of patch-level calculations in improving the performance of \awRe.

\subsection{Different k for look-up table}
% 在本节中,为了研究聚类个数对算法表现的影响,我们分别选取了不同的K,来生成查找表,并比较重用模型的效果. 我们使用NAS作为SR 模型,并将放大倍数设为4.
% 如图所示,随着K 的增加,需要重新微调的模型数量不断减少,但是重用模型的表现却增长.这说明聚类可以提升算法判断视频相似性的准确性,选择合适的聚类数量,可以降低训练开销以及选择重用模型的准确性
This ablation study investigates the impact of the number of clusters in Algorithm \ref{alg.model_encoder} on the performance of \awRe. We select different values of $K$ to generate different look-up tables on the \emph{Part1} of \emph{GVSET} and compare the performance of retrieval models on the \emph{Part2} of \emph{GVSET}. We use NAS\cite{yeo2018NAS} as the backbone with an upscaling factor of 4. As shown in \autoref{fig.dif_k.num}, the number of video segments requiring fine-tuning decreases as $K$ increases. An inflection point is observed when $K$ equals 10. The performance of the retrieval models improves when $K$ increases from 1 to 5 and stabilizes after $K$ reaches 5. The increase in $K$ results in more precise cluster centers, leading to the more specific encoding of SR models according to Algorithm \ref{alg.model_encoder}. This specific encoding enhances the accuracy during model retrieval. However, continuously increasing $K$ does not indefinitely yield benefits. A larger $K$ implies a need for more storage space and a higher retrieval overhead for the look-up table. Choosing an appropriate $K$ to cluster can reduce training overhead and improve the accuracy of selecting retrieval models.

\begin{figure}
  \centering
  \begin{minipage}[c]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/dif_k.pdf}
    \subcaption{Num of fine-tuning SR model}
    \label{fig.dif_k.num}
  \end{minipage}
  \begin{minipage}[c]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/dif_k_Dota2.pdf}
    \subcaption{PSNR of Dota2}
    \label{fig.dif_k.dota2}
  \end{minipage}  
  \\
  % \vspace{1em} % Adjust the space between the rows if needed
  \begin{minipage}[c]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/dif_k_H1Z1.pdf}
    \subcaption{PSNR of H1Z1}
    \label{fig.dif_k.h1z1}
  \end{minipage}
  \begin{minipage}[c]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/dif_k_PU.pdf}
    \subcaption{PSNR of PU}
    \label{fig.dif_k.pu}
  \end{minipage}
  \caption{(a) the number of fine-tuned models with different values of $k$. (b)-(d) the performance of \awRe~ on different games with different values of $k$}.
  \label{fig.dif_k}
\end{figure}

==> insight.tex <==
% 为了解决现有超神经增强视频传输在性能和训练开销的方面的不足,我们提出了全新的内容感知重用视频传输框架.
% {\color{red} sys overvirew, what challenges need to solve}

% We propose a novel cloud gaming transmission framework via content-aware retrieval, \awRe, to address the shortcomings of existing frameworks in training costs and performance.

% However, how to retrieve well-trained SR models from the model zoo for different video segments is a pressing challenge that needs to be addressed. In addition, We want to minimize the search cost as much as possible to meet the real-time requirements. The key insights of \awRe~ are encoding the SR model to construct the lookup table and retrieving the most suitable model for current video streaming from the lookup table. Achieving our goal requires redesigning major components of video delivery. This section describes the key design choices we make to overcome practical challenges.

In order to reuse fine-tuned SR models, some pressing challenges need to be solved, including model organization, online scheduler, and transfer strategy. This section describes the key design choices we make to overcome practical challenges.

\subsection{How to organize the model zoo?}
% 想要实现高效的管理,首先要实现对模型的标识.文章[]指出可以利用视频流自带的标签进行分类重用,但是对于云游戏来说即使是同一游戏也可能画面存在较大差异.如何组织并表示这些拟合不同冗余的模型成为一个仍待解决的问题.
\noindent\textbf{Key Challenge.} To achieve efficient and accurate model retrieval, it is essential to identify what
kind of videos an SR model is good at first. Existing approaches ~\cite{yao2017awDNN} suggest that video labels (such as Games, Athletics, and so on) can be used. However, the issue is that labels may be missing, or it is difficult to obtain labels. Besides, as shown in \autoref{fig.delay_hit_psnr}, there can be diversity even within the same game. Organizing and representing these models that fit different videos remains unresolved.

% 为了克服以上挑战,我们提出了模型查找表的方法.内容感知的模型可以看作是一种视频压缩算法。我们可以认为其捕获在大时间尺度上发生的冗余(例如多个GOPs),并在推理时对这些细节进行恢复.通过将视频段以及拟合视频段的超分辨模型转换成表中的键值对来实现对模型库的高效查找.

% 然而, 视频段无法被有效的检索,我们需要设计高效的编码方法.受到视频编码算法(h264等)对冗余信息压缩的启发,我们将帧切分成更小的补丁(block),使用预训练模型计算特征并对补丁特征进行聚类.使用聚类中心作为视频流的编码以实现对视频流进行编码的目的.查找表的组成如下
\noindent\textbf{Content-aware encoder.} To overcome these challenges, We propose a model lookup table comprising models and their encoding. Because the SR model can capture redundancies occurring in the video segment, we can design an appropriate feature extraction algorithm to encode the model based on the segment. Inspired by video coding algorithms (such as H.264\cite{sullivan2005h264}), we propose compressing information through clustering. First, we decode the video chunk $V_{i}$ and divide frames into smaller patches whose size is $w$ x $h$. Then, we cluster these patches based on the feature computed by the pre-trained classification model with K-means. The cluster centers $\{\mu_{i}^{0},...,\mu_{i}^{K-1}\}$ are used to identify the SR model $M_{i}$ in the lookup table. In summary, the composition of the lookup table is as follows:
\begin{equation}
\centering
    T_{i} \leftarrow < \{\mu_{i}^{0},...,\mu_{i}^{K-1}\}, M_{i}> 
    % \{\mu_{i}^{0},...,\mu_{i}^{K-1}\} = \{Encoder(P_{n})|P_{n} \in dataset_{M_{i}}\} 
\label{eq.model_look-up_table}
\end{equation}

where $T_{i}$ is the item of the look-up table, the model trained on the video segment $V_{i}$ is denoted as $M_{i}$ and $\{\mu_{i}^{0},...,\mu_{i}^{K-1}\}$ represents the encoding of $M_{i}$, as detailed
in Algorithm \ref{alg.model_encoder}.

% 图展示了在FIFA17的单帧图片上进行分类的结果.我们将图片切分成大小相同的补丁,并且使用resnet18计算补丁向量.对补丁的向量使用kmeans进行聚类(聚类个数取3).可以发现,背景部分(足球场)被分为一类,看台上的观众被分为另一类,剩下的部分(球员等)被归为一类. 在awRe中,我们通过聚类实现了对冗余信息的压缩,并保留了图像的内容特征.我们认为,这种内容感知的编码方式可以应用于应用于一系列(具有相似内容)视频,而不仅限于云游戏.
\autoref{fig.cluster_patch} shows the results of categorizing a single frame from FIFA17 using this solution. We divide the image into patches of equal size (e.g., 1080p is divided into 128x128 patches) and use ResNet18 to compute patch embedding. Then, We applied k-means clustering with three cluster centers. \autoref{fig.cluster_patch.1} represents the original picture. \autoref{fig.cluster_patch.2} illustrates the results after classification, with different colors indicating categories. It can be observed that the background (such as the football field) is grouped into Class 1, the audience on the stands is categorized into Class 3, and the remaining parts (such as football players) are assigned to Class 2. We believe this content-aware encoding approach can be applied to a series of videos with similar content and is not limited to cloud gaming.

\begin{figure}[htbp]
    % \centering
    \begin{minipage}[b]{0.48\linewidth}  
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{fig/FIFA17.1.png}
        \vspace{1pt}
        \subcaption{Original frame.}
        \label{fig.cluster_patch.1}
    \end{minipage} 
    \begin{minipage}[b]{0.48\linewidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{fig/cluster_patch_3.pdf}
        \subcaption{Classification mask.}
        \label{fig.cluster_patch.2}
    \end{minipage}
    \caption{Separability of different regions. (a) The original frame of FIFA17. (b) Different regions are divided into different groups according to our approach.}
    \label{fig.cluster_patch}
    % Visualization results of the classification.
    % Separability of different regions for a single frame
\end{figure}

\subsection{How to retrieve the optimal model?}
\label{sec.insight.choose_model}
% 对在线视频流,如何从模型库中选择重用模型直接影响用户的Qos,如果选择了不匹配的模型,可能导致灾难性的性能下降.同时,为了满足实时性的要求,调度算法的执行延迟应尽可能的小.
\noindent\textbf{Key Challenge.} For online video streams, how to choose the optimal SR model from the model lookup table directly impacts the user's Quality of Service (QoS) as mentioned in \autoref{fig.pre_exp_with_generic}. It is necessary to determine the best SR model for each frame because of the diversity of cloud gaming. Choosing a mismatched model can lead to catastrophic performance degradation. At the same time, to meet real-time requirements\cite{shi2011mobile,meilander2014mobile}, the execution delay of the scheduling algorithm should be minimized as much as possible.

% 分类模型对于相似图片生成的特征向量也是相近的,我们采用余弦相似度作为特性向量距离的度量.
% 通过计算补丁的特征向量与查找表中键值的距离,为每个补丁查询一个最佳模型. 一帧画面可以被切分成多个补丁,而每个补丁所命中的模型都可能不一样.为防止客户端执行图像增强的切换开销过大, 补丁再通过投票选出每帧的最佳公共模型.
\noindent\textbf{Online scheduler.} We aim to retrieve the model that was fine-tuned on the data similar to the current scene. According to \cite{wan2014deep,wang2014learning,van2020scan}, the pre-trained classification model we use in Algorithm \ref{alg.model_encoder} generates similar feature vectors for similar images. We use cosine similarity to measure the distance between feature vectors. We divide the current frame, denoted as $F_{i}$, into multiple patches, $\mathcal{D} = \{P_n\}_0^{N-1}$, where $N$ is the total number of patches in the frame. We query the optimal model for each patch from the lookup table according to \autoref{eq.quary}.
\begin{equation}
\centering
\begin{cases}
    Q(P_{n}) = \arg\max_{j}S_c(embedding_n,\mu_j^k) \\
    j \in (0,...,R-1), k \in (0,...,K-1)
    \label{eq.quary}
\end{cases}
\end{equation}
where the cosine similarity is denoted as $S_{c}$, the feature of n-th patch is represented as $embedding_n$ and $\mu_j^k$ is the k-th dimension of the $M_j$'s encoding. $K$ is the number of cluster centers, and $R$ is the number of SR models in the look-up table. In the worst case, each patch may hit a different model. We use the plurality voting algorithm to select the best common model for each frame based on the patches to prevent excessive switching costs for image enhancement at the client. 

% 在实际中,一帧的补丁总数较大(一个1080p可以被拆分成170个128x128的补丁). 然而,不是所有补丁都需要被过拟合,总的来说，越简单的图片在针对性训练后带来的收益越低，针对性训练在复杂的图片的收益更高,具体实验见8.1节.为了降低算法的计算开销,我们使用边缘检测对补丁进行剪枝.剩余的补丁如下
% 在处理在线视频流时,如果投票的获胜方获得绝大多数票数, 我们可以认为现有模型库已经可以较好的拟合当前帧.反之,则需要对当前视频流进行微调并加入模型库.
In practice, the $N$ is probably too large to increase computational overhead (e.g., a 1080p frame can be split into 170 patches of size 128x128). However, not all patches need to be overfitted. In general, the benefits from targeted training are lower for simpler patches and higher for more complex patches, as demonstrated in the experiments of Section \ref{sec.patch_pruning}. To reduce the computational cost of the algorithm, we use the score of edge detection\cite{chen2022arm} to prune the patches. The remaining patches are as follows.
\begin{equation}
    \hat{\mathcal{D}} = \{P_{i}|e_{i} > \lambda,P_{i} \in \mathcal{D}\}
    \label{eq.edge_filter}
\end{equation}
where $e_{i}$ is the edge score of the i-th patch and $\lambda$ is the threshold. The model to be retrieved for the current frame $F_{i}$ is
\begin{equation}
    M_{F_{i}} = \{M_{j} |j = V_p(Q(P_{n})), P_{n} \in \hat{\mathcal{D}} \} 
    \label{eq.frame_voting}
\end{equation}
where $V_{p}$ is the plurality voting algorithm. However, the SR model retrieved may not meet the image restoration requirements, such as low similarity between videos, especially in the unseen scene. To address this challenge, we assume if the winning candidate receives the vast majority of votes, the SR model retrieved can enhance the current frame well. On the contrary, we execute offline fine-tuning for the video stream and add the model to the repository by Algorithm \ref{alg.model_encoder}. More details of this method can be found in Algorithm \ref{alg.online_schedluer}.

\subsection{How to trade-off between video streams and model requests?}
\label{sec.insight.trade-off}
% 因为awRe会对每帧计算合适的重用模型,客户端必须从服务端下载SR模型后,再进行相应的图像增强.然而SR模型的下载请求会和视频流的传输竞争带宽.当客户端无法取得匹配的SR模型,会导致用户Qos的下降,反过来,如果下载模型占用了过多的带宽,也会导致视频流码率的降低.因为这种冲突关系的存在,如何平衡SR模型占用的带宽与图像增强效果需要我们认真的考量.

% Because \awRe~ calculates the appropriate reused model for each frame.

\noindent\textbf{Key Challenge.} The client must download the SR model from the server and execute the image enhancement locally.   In practice, the download request for the SR model competes with the bandwidth for video stream transmission. On the one hand, if downloading the model consumes too much bandwidth, it can reduce the video stream bitrate\cite{yeo2018NAS}. On the other hans, video quality will decrease when the client cannot obtain the optimal SR model \awRe~ recommends. Due to this conflicting relationship, careful consideration is required to balance the bandwidth occupied by the SR model and the image enhancement effect.

% 为了解决带宽占用问题,已有的做法是让一个SR 模型编码一个视频端.视频段越长,SR模型的带宽收益越高.
% 一段10s的30帧的视频流,在如果原视频为1080P,压缩后的视频为240P的条件下,如果想实现带宽压力的降低,最多可分配0.8Mbps的带宽传输模型.
% \noindent\textbf{Prefetching strategy.} The bandwidth allocated to the model stream is limited, and the maximum bandwidth of downloading models is shown as \autoref{eq.saved_bandwidth}. The greater the difference in bitrate before and after video stream compression, the higher the bandwidth can be allocated to download SR models. 
% \begin{equation}
%     \Delta_{bandwidth} = B_{hr} - B_{lr}
%     \label{eq.saved_bandwidth}
% \end{equation}
% where $B_{hr}$ and $B_{lr}$ are the bitrate of high-resolution and low-resolution cloud game video streaming. According to \cite{YouTube_encoding}, under the condition that the original video is 1080p and the compressed video is 270p, a maximum of 7 Mbps bandwidth can be allocated for model transmission.


\noindent\textbf{Prefetching strategy.} The bandwidth allocated to the model stream is limited, and the maximum bandwidth of downloading models is shown as $ \Delta_{bandwidth} = B_{hr} - B_{lr}$, where $B_{hr}$ and $B_{lr}$ are the bitrate of high-resolution and low-resolution cloud game video streaming. The greater the difference in bitrate before and after video stream compression, the higher the bandwidth can be allocated to download SR models. According to \cite{YouTube_encoding}, under the condition that the original video is 1080p and the compressed video is 270p, a maximum of 7 Mbps bandwidth can be allocated for model transmission.

% 对于awRe,不同帧可能会命中不同的SR模型,导致最高40Mbps的模型下载带宽占用. 而如果让一个模型处理一系列帧可能会导致性能的下降.为克服这个挑战,我们提出预取的缓存策略.因为视频流在时间上存在一定的相似性,当当前帧命中模型时,我们选择将其相邻的多个模型一起发送给客户端.我们将从模型1转移到模型2的概率定义为
% 对于客户端已经下载的SR模型,我们使用LUR算法维持本地队列
However, different frames may request different SR models according to Algorithm \ref{alg.online_schedluer}, leading to a maximum model download bandwidth utilization of up to 40 Mbps. That is 6 times the maximum model bandwidth. However, having an SR model handle the entire video segment may decrease enhancement quality. Fortunately, because of the certain similarity in the temporal aspect of video streams, when the current frame hits $M_{i}$, there is a high probability of $M_{j}$, which is similar to $M_{i}$. Based on this, we propose the prefetching strategy to minimize the impact of model transmission on the latency of cloud game video streaming. We choose to send a set of SR model $\Omega = \{M_{i},..., M_{j}\}$ to the client together in which there is a high probability of $M_{j}$ hitting after $M_{i}$. We let this series of models $\Omega = \{M_{i},..., M_{j}\}$ process the video segment.

We define the probability of transitioning from $M_{i}$ to $M_{j}$ as $p_{i,j}$ that is calculated by \autoref{eq.transfer_matrix}. The higher the transition probability, the more similar the models.
\begin{equation}
\centering
\begin{cases}
    p_{i,j} = softmax(d_{i,j}) \\
    d_{i,j} = \sum_{k=0}^{K-1}\max(d_{i,j}^k) \\
    d_{i,j}^k = \{S_c(\mu_i^k,\mu_j^{\hat{k}})|\hat{k} \in \{0,1,...,K-1\}\}\\
    j \in \{0,1,...,R-1\}
\end{cases}
\label{eq.transfer_matrix}
\end{equation}
Cosine similarity is denoted as $S_{c}$. $\mu_i^k$ is the k-th dimension of $M_{i}$'s encoding calculated by Algorithm \ref{alg.model_encoder}. $K$ is the number of cluster centers, and $R$ is the number of SR models in the look-up table. For the SR models already downloaded by the client, we use the Least Recently Used (LRU) algorithm to maintain a local cache, as detailed in Algorithm \ref{sec.sys.prefetching_cache}.

% 



